DiMSUM: Diffusion Mamba -- A Scalable and Unified Spatial-Frequency Method for Image Generation

We introduce a novel state-space architecture for diffusion models, effectively harnessing spatial and frequency information to enhance the inductive bias towards local features in input images for image generation tasks. While state-space networks, including Mamba, a revolutionary advancement in recurrent neural networks, typically scan input sequences from left to right, they face difficulties in designing effective scanning strategies, especially in the processing of image data. Our method demonstrates that integrating wavelet transformation into Mamba enhances the local structure awareness of visual inputs and better captures long-range relations of frequencies by disentangling them into wavelet subbands, representing both low- and high-frequency components. These wavelet-based outputs are then processed and seamlessly fused with the original Mamba outputs through a cross-attention fusion layer, combining both spatial and frequency information to optimize the order awareness of state-space models which is essential for the details and overall quality of image generation. Besides, we introduce a globally-shared transformer to supercharge the performance of Mamba, harnessing its exceptional power to capture global relationships. Through extensive experiments on standard benchmarks, our method demonstrates superior results compared to DiT and DIFFUSSM, achieving faster training convergence and delivering high-quality outputs. The codes and pretrained models are released at https://github.com/VinAIResearch/DiMSUM.git.

==> acknowledgement.tex <==
\section*{Acknowledgements}
Research partially funded by research grants to Prof. Dimitris Metaxas from NSF: 2310966, 2235405, 2212301, 2003874, 1951890, AFOSR 23RT0630, and NIH 2R01HL127661.

==> tabs/abl_freq_step.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{l c c c c c}
    \toprule
     & FID$\downarrow$ & Recall$\uparrow$ & Params & GFLOPs \\ \hline
    DCT & 5.53 & 0.50 & 436M & 67.33 \\
    EinFFT & 5.63 & 0.48 & 371M & 66.96 \\
    \rowcolor{pink!60} Wavelet & 4.92 & 0.50 & 436M & 62.42 \\
    \midrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of frequency types. All experiments are evaluated at 250 epochs on CelebA-HQ  $256 \times 256$ dataset and no shared-transformer is used.}
    \label{tab:ab_frequency_type}
\end{table}

==> tabs/abl_fusion_layer.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l c c c c}
    \toprule
     & FID$\downarrow$ & Recall$\uparrow$ & Params & GFLOPs \\
    \toprule
    % Concat & & & & & & \\
    Linear & 6.00 & 0.47 & 411M & 60.83 \\
    Attention & 5.05 & 0.50 & 461M & 73.71 \\
    \rowcolor{pink!60} Cross-Attention fusion layer (swap q) & 4.92 & 0.50 & 436M & 67.27 \\
    Cross-Attention fusion layer (swap k) & 5.45 & 0.48 & 436M & 67.27 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of fusion layer. All experiments are evaluated at 250 epochs on CelebA-HQ $256 \times 256$ dataset and no globally-shared transformer is used.}
    \label{tab:ab_fusion_layer}
\end{table}

==> tabs/abl_network_components.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{l c c c c c}
    \toprule
     & FID$\downarrow$ & Recall$\uparrow$ & Params & GFLOPs \\
    \toprule
    Baseline & 6.19 & 0.46 & 413M & 51.65 \\
    + Conditional Mamba & 5.27 & 0.49 & 446M & 51.69 \\
    + Wavelet Mamba (w/ concat) & 5.87 & 0.47 & 394M & 56.54 \\
    + Cross-Attention fusion layer & 4.92 & 0.50 & 436M & 62.42 \\
    \rowcolor{pink!60} + Globally-shared transformer block & 4.65 & 0.52 & 459M & 84.49 \\
    \midrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of our network components. All experiments are evaluated at epoch 250 on CelebA-HQ  $256 \times 256$ dataset.}
    \label{tab:ab_network_comps}
\end{table}

==> tabs/abl_scanning.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{l c c c}
    \toprule
    Order & FID$\downarrow$ & Recall$\uparrow$ & iters/s $\uparrow$ \\
    \toprule
    \multicolumn{4}{c}{\textbf{Conditional Mamba Only}} \\
    \toprule
    % Uni & & & & \\
    Bi & 6.39 & 0.44 & 2.06 \\
    \rowcolor{pink!60} Sweep-4 & 5.27 & 0.49 & 2.06 \\
    Sweep-8 & 5.53 & 0.48 & 1.97 \\
    Zigzag-8 & 6.17 & 0.46 & 1.97 \\
    Jpeg-8 & 6.26 & 0.45 & 1.97 \\
    Window & 10.88 & 0.36 & 2.05 \\
    % \midrule
    % \multicolumn{5}{c}{\textbf{Wavelet Mamba only}} \\
    % \midrule
    % Sweep-4 &  &  & & \\
    % Window & 23.80 & 0.59 & 0.19 & 1.72 \\
    \midrule
    \multicolumn{4}{c}{\textbf{Spatial-frequency Mamba}} \\
    \midrule
    Sweep-4 | Sweep-4 & 5.41 & 0.49 & 1.54 \\
    \rowcolor{pink!60} Sweep-4 | Window & 4.92 & 0.50 & 1.54 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of scanning orders. Here, we keep it simple by using only Mamba block for all experiments without the globally-shared transformer and fusion layer. In Spatial-frequency Mamba, we use "Sweep-4" scanning for spatial features by default and only test other scanning methods for wavelet features.} 
    \label{tab:scanning_orders}
\end{table}

==> tabs/abl_transform_layer.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{l c c c c}
    \toprule
     & FID$\downarrow$ & Recall$\uparrow$ & Params & GFLOPs \\
    \toprule
    \multicolumn{5}{c}{\textbf{Conditional Mamba}} \\
    \toprule
    Globally-shared & 5.40 & 0.49 & 469M & 78.30 \\
    \toprule
    \multicolumn{5}{c}{\textbf{Spatial-Frequency Mamba}} \\
        \toprule
    Independent & 5.08 & 0.49 & 397M & 63.37 \\
    \rowcolor{pink!60} Globally-shared & 4.65 & 0.52 & 459M & 84.49 \\
    
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of transformer layer. All experiments are evaluated at 250 epochs on CelebA-HQ $256 \times 256$ dataset.}
    \label{tab:ab_transformer}
\end{table}


==> tabs/abl_wavelet_lvl.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{l c c c}
    \toprule
    \#Lv & FID$\downarrow$ & Recall$\uparrow$ & GFLOPs \\ \hline
    1 & 5.09 & 0.50 & 84.48 \\
    \rowcolor{pink!60} 2 & 4.65 & 0.52 & 84.49 \\
    3 & 5.23 & 0.49 & 84.50 \\
    \midrule
    \end{tabular}
    \vspace{2mm}
    \caption{Ablation of wavelet levels. All experiments are evaluated at 250 epochs on CelebA-HQ  $256 \times 256$ dataset.}
    \label{tab:ab_wavelet_lv}
\end{table}

==> tabs/app_hyperparam.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \caption{Hyper-parameters of our DiMSUM network.}
\begin{tabular}{lccc}
\toprule
              & Celeb-A       & Church & ImageNet      \\ \midrule
Learning rate   & $1\text{e-4}$ & $1\text{e-}4$                                         & $1\text{e-}4$ \\
$\beta_1,\beta_2$         & 0.9, 0.999    & 0.9, 0.999                                            & 0.9, 0.999    \\
Batch size    & 64            &                                                       & 704           \\
Droppath      & 0.1           & 0.2                                                   & 0.1           \\
Max-grad-norm & 2             & 2                                                     & 1             \\
Label-dropout & 0.            & 0.                                                    & 0.15          \\
Epochs        & 250           & 300                                                   &               \\
GPUs          & 2             &                                                       & 8             \\
Train days    & 0.89          &                                                       &               \\ \bottomrule
\end{tabular}
    \label{tab:hyperparams}
\end{table}

==> tabs/app_network_config.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \caption{DiMSUM network config.}
\begin{tabular}{lc}
\toprule
Config                  & \multicolumn{1}{l}{Value} \\ \midrule
Depth                   & 16                        \\
Hidden size             & 1024                      \\
Patch size              & 2                         \\
\begin{tabular}[c]{@{}l@{}}Use learnable absolute\\ positional embedding\end{tabular} & True \\
Attention every k layer & 4                         \\ \bottomrule
\end{tabular}
    \label{tab:dimsum_config}
\end{table}


==> tabs/celeb256.tex <==
\begin{table}
\centering
\small
    \begin{tabular}{l c c c c}
        \toprule
        Model & NFE$\downarrow$ & FID$\downarrow$ & Recall$\uparrow$  & Epochs \\
        \midrule
        % \multicolumn{6}{c}{\textbf{CelebA-HQ 256}} \\
        % \midrule
        Ours & 61 & \textbf{4.62} & \textbf{0.52} & \textbf{250} \\
        Zigma{\textdagger} \cite{hu2024zigma}  & 250 & 7.66 & 0.40 & 400 \\
        % Zigma & 250 & 6.17 & 0.46 & \\
        % LFM-8 (ADM) & 85 & 5.67 & \textbf{0.78} & 0.43 & 3.42 \\
        % FM \cite{lipman2023flow}* &128 & 7.34 & - & - & -\\
        \midrule
        LFM-8 \cite{dao2023flow} & 89 & 5.26 & 0.46 & 500 \\
        LDM-4 (ADM) \cite{rombach2022high} & 500 & 5.11 & 0.49 & 600 \\
        LDM-8 (ADM)\textdaggerdbl & 250 & 15.37 & - & 500 \\
        LDM-8 (DiT)\textdaggerdbl & 250 & 10.21 & - & 500 \\
        \midrule
        LSGM \cite{vahdat2021scorebased} & 23 & 7.22 & -& 1K \\
        WaveDiff \cite{phung2023wavediff} & 2 & 5.94 & 0.37 & 500 \\
        DDGAN \cite{xiao2021tackling} & 2 & 7.64 & 0.36 & 800 \\
        RDGAN \cite{dao2023robust} &2 &5.60 &0.38 & - \\
        Score SDE \cite{song2020score} & 4000 & 7.23 & - & ~6.2K \\
        StyleSwin \cite{zhang2022styleswin} & 1 & 3.25 & - & ~30K \\
        % \midrule
        % \multicolumn{6}{c}{\textbf{CelebA-HQ 512}} \\
        % \midrule
        % LFM-8 (ADM) & 94 & \textbf{6.35} & \textbf{0.77} & \textbf{0.41} & 5.13 \\
        % WaveDiff \cite{phung2023wavediff} & 2 & 6.40 & - & 0.35 & 0.59 \\
        % DDGAN \cite{xiao2021tackling} & 2 & 8.43 & - & 0.33 & 1.49 \\
        
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Quantitative result of our method versus others on CelebA-HQ $256 \times 256$ dataset. {\textdagger} is our reproduced result based on Zigma's official code and {\textdaggerdbl} is an adopted result from LFM \cite{dao2023flow}.}
    \label{tab:celeb256}
\end{table}

==> tabs/celeb512.tex <==
\begin{table}

\centering
\small
    \begin{tabular}{l c c c c}
        \toprule
        Model & NFE$\downarrow$ & FID$\downarrow$ & Recall$\uparrow$ &Epochs\\
        \midrule
        % \multicolumn{5}{c}{\textbf{CelebA-HQ 512}} \\
        % \midrule
        Ours & 250 & \textbf{6.08} & \textbf{0.46} &\textbf{175}\\
        \midrule
        LFM-8 \cite{dao2023flow} & 94 & 6.35 & 0.41  & 500 \\
        % LFM-8 \cite{dao2023flow} & 250 & 6.36 & 0.41 &  &\\
        WaveDiff \cite{phung2023wavediff} & 2 & 6.40 & 0.35  & 400 \\
        DDGAN \cite{xiao2021tackling} & 2 & 8.43 & 0.33  & 400 \\
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Quantitative result of our method versus others on CelebA-HQ $512 \times 512$ dataset. }
    \label{tab:celeb512}
\end{table}

==> tabs/imgnet256_iters_final.tex <==

% \begin{table}[t]
\begin{wraptable}{rh}{6.5cm}
    \vspace{-12mm}
    \centering
    \vspace{2mm}
    \caption{Class-conditional image generation on ImageNet $256 \times 256$ dataset.}
    \normalsize
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c}
        \toprule
    Model & FID$\downarrow$ & Recall$\uparrow$ & Params & \#Iters $\times$ Bs & Epoch \\
    \midrule
    % Ours (ADM) & 16.71 & 0.56 & 387M \\
    % + cfg=1.25 & 8.58 & 0.50 & 387M \\
    % Ours (DiT B/2) & 24.99 & 0.37 & 130M \\
    % + cfg=1.5 & 5.76 & 0.34 & 130M \\
    Ours &\textbf{8.61} &\textbf{0.67} & 460M & 936K $\times$ 704 &510\\
    % Ours-G (cfg=1.5) &2.32 &0.57 & 460M & 2550K \times 704 \\
    Ours-G &\textbf{2.11} &\textbf{0.59} & 460M & 936K $\times$ 704 &510\\ \midrule
    SSM-based \\    
    % DiS-H/2 \cite{fei2024dis} (cfg=1.5) & 2.10 & 0.56 & 900M & 1.0K \\
    DIFFUSSM-XL \cite{yan2024diffusion} & 9.07 & 0.64 & 673M & 2578K$\times$ 256 &515 \\
    DIFFUSSM-XL-G & 2.28 & 0.56 & 673M & 2578K $\times$ 256 &515 \\
    \midrule
    % LFM (DiT B/2) & 20.38 & 0.56 & 130M & 900 \\
    % LFM (DiT B/2, cfg=1.25) & 8.77 & - & 0.48 & 130M & 900 \\
    % LFM (DiT B/2, cfg=1.5) & 4.46 & 0.42 & 130M & 900 \\
    % LDM-8 \cite{rombach2022high} & 15.51 & 0.63 & 395M & 240 \\
    % LDM-8-G & 7.76 & 0.35 & 506M & 240 \\
    UNet-based \\
    LDM-4 \cite{rombach2022high} & 10.56 & 0.62 & 400M & 178K $\times$ 1200 &200\\
    LDM-4-G & 3.60 & 0.48 & 400M & 178K $\times$ 1200  &200\\
    \midrule
    % DiT-B/2 \cite{Peebles2022DiT} & 43.47 & - & - & 130M \\
    % Ours &15.29 & - &460M &80 \\
    Transformer-based \\
    DiT-L/2 \cite{Peebles2022DiT} & 23.33 & - & 458M & 400K $\times$ 256 &80 \\
    % DiT-XL/2 & 19.47 & - & 675M & 80 \\
    DiT-XL/2 & 9.62 & 0.67 & 675M & 7000K $\times$ 256 &1.4K\\
    % DiT-XL/2-G (cfg=1.25) & 3.22 & 0.62 & 675M & 1.4K \\
    DiT-XL/2-G & 2.27 & 0.57 & 675M & 7000K $\times$ 256 &1.4K\\
    SiT-XL/2 \cite{ma2024sit} & 9.40 & - & 675M & 7000K $\times$ 256 &1.4K\\
    SiT-XL/2-G & 2.15 & 0.59 & 675M & 7000K $\times$ 256 &1.4K \\
    % SiT-XL/2 (SDE) & 8.60 & - & 675M & 1.4K \\
    % SiT-XL/2-G (cfg=1.5, SDE) & 2.06 & 0.59 & 675M & 1.4K \\
    
    % \midrule
    % ADM \cite{dhariwal2021diffusion} & 10.94 & 0.63 & 554M & 400 \\
    % ADM-U & 7.49 & 0.63 & 554M & 400 \\
    % ADM-G & 4.59 & 0.52 & 608M & 400 \\
    % ADM-G, ADM-U & 3.94 & 0.53 & - & 400 \\
    % \midrule
    % CDM \cite{ho2022cdm} & 4.88 & - & - & 2.2K \\
    % \midrule
    % ImageBART \cite{esser2021imagebart} & 7.44 & - & 3.5B \\
    % \midrule
    % VQGAN+T \cite{esser2021taming} & 5.88 & - & 1.3B \\
    % MaskGIT \cite{chang2022maskgit} & 6.18 & 0.51 & 227M & 280 \\
    % RQ-Transformer \cite{lee2022autoregressive} & 3.80 & - & 3.8B & - \\
    % \midrule
    \midrule
    GAN model \\
    BigGan-deep \cite{brock2018large} & 6.95 & 0.28 & 160M & - \\
    StyleGAN-XL \cite{sauer2022stylegan} & 2.30 & 0.53 & 166M & 25000K $\times$ 256 & 4K \\
    % GigaGAN \cite{kang2023gigagan} & 3.45 & 0.61 & 569M & \\
    \bottomrule
    \end{tabular}}
    \vspace{-1mm}
    \label{tab:full_imagenet}
% \end{table}
    \vspace{-1mm}
\end{wraptable}

% \begin{table}[t]
%     % \vspace{-1mm}
%     \centering
%     \caption{Class-conditional image generation on ImageNet $256 \times 256$ dataset.}
%     % \vspace{-2mm}
%     \scriptsize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{l c c c c}
%         \toprule
%     Diffusion model & FID$\downarrow$ & Recall$\uparrow$ & Params & \#Iters \\
%     \midrule
%     % Ours (ADM) & 16.71 & 0.56 & 387M \\
%     % + cfg=1.25 & 8.58 & 0.50 & 387M \\
%     % Ours (DiT B/2) & 24.99 & 0.37 & 130M \\
%     % + cfg=1.5 & 5.76 & 0.34 & 130M \\
%     Our submission results \\
%     Ours & 9.47 & 0.65 & 460M & 1600K \\
% Ours-G & 2.26 & 0.56 & 460M & 1600K \\
    
%     \midrule
%     Our longer training results \\
%     Ours &\textbf{8.61} &\textbf{0.67} & 460M & 
% 2550K \\
%     % Ours-G (cfg=1.5) &2.32 &0.57 & 460M & 2550K \times 704 \\
%     Ours-G &\textbf{2.11} &\textbf{0.59} & 460M & 2550K \\ \midrule
%     SSM-based \\    
%     % DiS-H/2 \cite{fei2024dis} (cfg=1.5) & 2.10 & 0.56 & 900M & 1.0K \\
%     DIFFUSSM-XL & 9.07 & 0.64 & 673M & 2578K \\
%     DIFFUSSM-XL-G & 2.28 & 0.56 & 673M & 2578K \\
%     \midrule
%     % LFM (DiT B/2) & 20.38 & 0.56 & 130M & 900 \\
%     % LFM (DiT B/2, cfg=1.25) & 8.77 & - & 0.48 & 130M & 900 \\
%     % LFM (DiT B/2, cfg=1.5) & 4.46 & 0.42 & 130M & 900 \\
%     % LDM-8 \cite{rombach2022high} & 15.51 & 0.63 & 395M & 240 \\
%     % LDM-8-G & 7.76 & 0.35 & 506M & 240 \\
%     UNet-based \\
%     LDM-4 & 10.56 & 0.62 & 400M & 178K \\
%     LDM-4-G & 3.60 & 0.48 & 400M & 178K \\
%     \midrule
%     % DiT-B/2 \cite{Peebles2022DiT} & 43.47 & - & - & 130M \\
%     % Ours &15.29 & - &460M &80 \\
%     Transformer-based \\
%     DiT-L/2 & 23.33 & - & 458M & 400K \\
%     % DiT-XL/2 & 19.47 & - & 675M & 80 \\
%     DiT-XL/2 & 9.62 & 0.67 & 675M & 7000K \\
%     % DiT-XL/2-G (cfg=1.25) & 3.22 & 0.62 & 675M & 1.4K \\
%     DiT-XL/2-G & 2.27 & 0.57 & 675M & 7000K \\
%     SiT-XL/2 & 9.40 & - & 675M & 7000K \\
%     SiT-XL/2-G & 2.15 & 0.59 & 675M & 7000K \\
%     % SiT-XL/2 (SDE) & 8.60 & - & 675M & 1.4K \\
%     % SiT-XL/2-G (cfg=1.5, SDE) & 2.06 & 0.59 & 675M & 1.4K \\
    
%     % \midrule
%     % ADM \cite{dhariwal2021diffusion} & 10.94 & 0.63 & 554M & 400 \\
%     % ADM-U & 7.49 & 0.63 & 554M & 400 \\
%     % ADM-G & 4.59 & 0.52 & 608M & 400 \\
%     % ADM-G, ADM-U & 3.94 & 0.53 & - & 400 \\
%     % \midrule
%     % CDM \cite{ho2022cdm} & 4.88 & - & - & 2.2K \\
%     % \midrule
%     % ImageBART \cite{esser2021imagebart} & 7.44 & - & 3.5B \\
%     % \midrule
%     % VQGAN+T \cite{esser2021taming} & 5.88 & - & 1.3B \\
%     % MaskGIT \cite{chang2022maskgit} & 6.18 & 0.51 & 227M & 280 \\
%     % RQ-Transformer \cite{lee2022autoregressive} & 3.80 & - & 3.8B & - \\
%     % \midrule
%     \midrule
%     GAN model \\
%     BigGan-deep & 6.95 & 0.28 & 160M & - \\
%     StyleGAN-XL & 2.30 & 0.53 & 166M & 25000K \\
%     % GigaGAN \cite{kang2023gigagan} & 3.45 & 0.61 & 569M & \\
%     \bottomrule
%     \end{tabular}
%     \vspace{-1mm}
%     \label{tab:full_imagenet}
% % \end{table}
%     % \vspace{-1mm}
% \end{table}

==> tabs/lsun256.tex <==
\begin{table}
\small
\centering
    \begin{tabular}{lcccc}
    \toprule
    Model & NFE$\downarrow$ & FID$\downarrow$ & Recall$\uparrow$ & Epochs \\ \midrule
    Our                                 & 250  & \textbf{3.76} & \textbf{0.56} & \textbf{395} \\
    DIFFUSSM \cite{yan2023diffusion}                           & 250  & 3.94          & -             & -   \\ \midrule
    LFM \cite{dao2023flow} (DiT L/2)                       & 250  & 5.54          & 0.48          & 500 \\
    % FM \cite{lipman2023flow}            & 250  & 10.54         & -             & -   \\
    LDM \cite{rombach2022high}          & 250  & 4.02          & 0.52          & 400 \\
    WaveDiff \cite{phung2023wavediff}   & 2    & 5.06          & 0.40          & 500 \\
    DDPM \cite{ho2020denoising}         & 1000 & 7.89          & -             & 640 \\
    % ImageBART \cite{esser2021imagebart} & 1000 & 7.32          & -             & -   \\ 
    \midrule
    StyleGAN \cite{karras2019style}     & 1    & 4.21          & -             & -   \\
    StyleGAN2 \cite{karras2020training} & 1    & 3.86          & 0.36          & 13K \\ \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{Quantitative result of our method versus others on LSUN Church $256 \times 256$ dataset.}
    \label{tab:lsun256}
\end{table}

% \begin{table}
% \small
% \centering
%     \begin{tabular}{l c c  c c c}
%         \toprule
%         Model  &NFE$\downarrow$ &FID$\downarrow$  &Recall$\uparrow$ & Time(s)$\downarrow$ & Epochs \\
%         \midrule
%         Our &250 &\textbf{3.76} &\textbf{0.56} & & 300 \\
%         DIFFUSSM & 250 & 3.94 & - & - & - \\
%         \midrule
%         % LFM (ADM) &250 & 7.7 & & 0.39 & 3.5 \\
%         LFM (DiT L/2) &250 & 5.54 & 0.48 & 1.67 & 500 \\
%         FM \cite{lipman2023flow}  &250 &10.54 & - &- & -\\
%         LDM \cite{rombach2022high} &250 & 4.02 & 0.52 & 3.79* & 400 \\
%         WaveDiff \cite{phung2023wavediff} &2 & 5.06  & 0.40 & 1.54 & 500 \\
%         DDPM \cite{ho2020denoising} &1000 & 7.89 & - & - & 640 \\
%         ImageBART \cite{esser2021imagebart} &1000 & 7.32 & - & - & - \\
%         \midrule
%         StyleGAN \cite{karras2019style} &1 & 4.21 & - & - &  - \\
%         StyleGAN2 \cite{karras2020training} &1 & 3.86 &0.36 & - & 13K \\
%         % ProjectedGAN \cite{Sauer2021NEURIPS} &1 & \textbf{1.59} & 0.44 & - & 5.3K \\
%         \bottomrule
%     \end{tabular}
%     \vspace{3mm}
%     \caption{Quantitative result of our method versus others on LSUN Church $256 \times 256$ dataset.}
%     \label{tab:lsun256}
% \end{table}



% \toprule
%     Model & FID$\downarrow$ & Recall$\uparrow$ & Time(s)$\downarrow$ \\
%     \midrule
%     Ours (ADM) & 7.05 & 0.39 & 5.42 \\
%     % Ours (DiT L/2) & 5.62 & 0.41 & 1.67 \\
%     Ours (DiT L/2) & 4.92 & 0.44 & 1.67 \\
    
%     \midrule
%     LDM \cite{rombach2022high} & 2.95 & 0.48 & 2.90* \\
%     DDPM \cite{ho2020denoising} & 4.9 & - & - \\
%     ImageBART \cite{esser2021imagebart} & 5.51 & - & - \\
%     ADM \cite{dhariwal2021diffusion} & \textbf{1.90} & \textbf{0.51} & - \\
%     \midrule
%     PGGAN \cite{karras2017progressive} &8.34 &- &-\\
%     StyleGAN \cite{karras2019style} & 2.35 & 0.48 & - \\
%     ProjectedGAN & 1.52 & 0.34 & - \\
%     DiffGAN \cite{wang2023diffusiongan} & \textbf{1.43} & \textbf{0.58} & - \\


==> tabs/supp_gflops.tex <==
\begin{table}
\centering
\small
\caption{Speed and GFLOPs comparison. Single-sample generation was performed, and all tests were conducted on an NVIDIA A100 40GB GPU.}
\vspace{2mm}
\begin{tabular}{lcccc}
\toprule
Method &	Time	& MEM & Params &	GFlops \\
\midrule
\multicolumn{5}{c}{256 (latent size: 
$32\times 32$)} \\
\midrule
Ours-L/2 &	2.20s	& 2.42G & 460M &	84.49 \\
DiT-L/2	& 3.80s & 2.30G	& 458M	& 80.74 \\
\midrule
\multicolumn{5}{c}{512 (latent size: 
$64\times 64$)} \\
\midrule
Ours-L/2	& 2.86s & 2.46G &	461M &	337.48 \\
DiT-L/2	& 4.78s & 2.34G &	459M &	361.14 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\label{tab:supp_speed_gflops}
\end{table}

==> tabs/supp_inference_speed.tex <==
\begin{table}
% \begin{wraptable}{r}{0.5\textwidth}
\centering
\small
\vspace{2mm}
\caption{Inference speed comparison between DiT-L/2 and our model to generate one $256\times256$ image, tested on NVIDIA A100 40GB GPU.}
\begin{tabular}{lcr}
 \toprule
Order\textbf{}  & \textbf{Latency} & \textbf{Params} \\ \midrule
DiT-L/2    & 3.8s             & 458M             \\
DiMSUM-L/2 & \textbf{2.2s}             & 460M \\
\bottomrule
\end{tabular}
\vspace{2mm}
\label{tab:supp_scanning_abinference_speed}
\end{table}
% \end{wraptable}

==> tabs/supp_lsun.tex <==
\begin{table}[t]
\small
\centering
\vspace{2mm}
\caption{Scaling DiMSUM's parameters on LSUN Church.}
\label{tab:supp_lsun}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{FID$\downarrow$} & \textbf{Epochs} & \multicolumn{1}{l}{\textbf{Params}} \\ \hline
DiMSUM-L/2                          & 3.76 & 395 & 460M \\
DiMSUM-XL/2                         & \textbf{3.45}          & 340 & 718M \\
DIFFUSSM    & 3.94          & -   & 673M \\ \hline
StyleGAN     & 4.21          & -   & -    \\
StyleGAN2 & 3.86          & 13K & -    \\ \bottomrule
\end{tabular}
\end{table}

==> tabs/supp_ode_vs_ddpm_solver.tex <==
\begin{table}

\centering
\small
    \begin{tabular}{l c c}
        \toprule
         & dopri5 & Euler/DDIM (250NFE) \\
        \midrule
        % \multicolumn{5}{c}{\textbf{CelebA-HQ 512}} \\
        % \midrule
        CelebA 256 & 4.62 & 4.65 \\
        Church 256 & 3.76 & 3.77 \\
        ImageNet 256-G & 2.11 & 2.12 \\
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \caption{FID50K of ODE solver and DDPM/DDIM solver on CelebA.}
    \label{tab:solver_comp}
\end{table}

==> tabs/supp_scanning_ab.tex <==
\begin{table}
\centering
\small
\caption{Additional ablation of scanning orders involves using window scanning for wavelet blocks and examining the sensitivity of DiMSUM to different scanning orders for spatial blocks. For simplicity, no shared-transformer block is used.}
\vspace{2mm}
\begin{tabular}{lcc}
 \toprule
Order & freq + spatial &spatial \\ \midrule
Bi & 5.47 & 6.39\\
Jpeg & 5.74 &6.26\\
sweep-8& 5.23&5.53 \\
zigma-8& 5.71&6.26 \\
sweep-4 & \textbf{4.92}&5.28 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\label{tab:supp_scanning_ab}
\end{table}
